UniHPE: Towards Unified Human Pose Estimation via Contrastive Learning

In recent times, there has been a growing interest in developing effective perception techniques for combining information from multiple modalities. This involves aligning features obtained from diverse sources to enable more efficient training with larger datasets and constraints, as well as leveraging the wealth of information contained in each modality. 2D and 3D Human Pose Estimation (HPE) are two critical perceptual tasks in computer vision, which have numerous downstream applications, such as Action Recognition, Human-Computer Interaction, Object tracking, etc. Yet, there are limited instances where the correlation between Image and 2D/3D human pose has been clearly researched using a contrastive paradigm. In this paper, we propose UniHPE, a unified Human Pose Estimation pipeline, which aligns features from all three modalities, i.e., 2D human pose estimation, lifting-based and image-based 3D human pose estimation, in the same pipeline. To align more than two modalities at the same time, we propose a novel singular value based contrastive learning loss, which better aligns different modalities and further boosts the performance. In our evaluation, UniHPE achieves remarkable performance metrics: MPJPE $50.5$mm on the Human3.6M dataset and PAMPJPE $51.6$mm on the 3DPW dataset. Our proposed method holds immense potential to advance the field of computer vision and contribute to various applications.

==> legacy/1_intro.tex <==
\section{Introduction}
\label{sec:intro}


Estimating 2D and 3D human poses from RGB images is one of the foundational tasks in the computer vision field, which can be further used for several downstream tasks like multiple object tracking\cite{andriluka2018posetrack, snower2020keytrack}, action recognition\cite{shahroudy2016nturgbd, duan2022pyskl}, human-computer interaction\cite{wang2018hci, hu2018vgpn}, human body reconstruction\cite{weng2022humannerf, li2023hybrik}, sports application\cite{zhao2023survey, jiang2022golfpose}, \etc. Previous works follow the paradigms which estimate 3D human pose from 2D human pose (so-called lifting)\cite{pavllo2019videopose3d, zhao2019semgcn, zheng2021poseformer} or 2D image directly\cite{kolotouros2019spin, sun2022BEV, sun2021ROMP}. The lifting process remains a two-stage paradigm heavily reliant on the efficacy of 2D human pose detectors in the initial phase, as direct estimation from 2D images grapples with challenges related to subpar performance and generalization capabilities. Regarding the architectures for lifting networks, initial efforts relied on networks utilizing fully connected layers\cite{martinez2017simplebaseline}, spatial-temporal convolution networks\cite{pavllo2019videopose3d}, graph neural networks\cite{zhao2019semgcn}, and transformer\cite{li2022transpose}. The networks are designed to learn the mapping from 2D poses to target 3D poses.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/intro.pdf}
    \caption{Aligned Image, 2D and 3D pose features in the feature space.}
    \label{fig:intro}
\end{figure}

% However, there are some challenges with data misalignment, such as {add more dataset description}. 

From the perspective of representation learning, previous methods have been dedicated to mapping the representation of RGB images or 2D poses into the corresponding 3D pose space. This brings up the question: \textit{Could we learn a shared Image-2D-3D human pose representation}? In this paper, we consider 3D human pose estimation as an Image-3D and 2D-3D feature alignment task, and 2D human pose estimation as an Image-2D feature alignment task. Inspired by CLIP\cite{radford2021clip}, which proposes to learn transferable visual features with natural language supervisions trained on web-scale image-text pairs data, we claim that RGB image, 2D and 3D human pose feature alignment and estimation tasks can also benefit from contrastive representation learning and large-scale dataset, \eg, Human3.6m\cite{ionescu2013h36m}, MPI-INF-3DHP\cite{mono-3dhp2017}. 

Learning joint embeddings across more than two modalities is a challenge. Girdhar \etal \cite{girdhar2023imagebind} propose IMAGEBIND, which aligns features across six modalities by training on naturally aligned pairs. Xue \etal \cite{xue2023ulip} align point cloud features to pre-trained text and image features from CLIP. In previous works, embeddings from different modalities are mainly aligned pairwisely, while the anchor encoders of one or two modalities are frozen during training. To align the images, 2D and 3D poses, three modalities, jointly, we propose a new loss that takes advantage of the singular value of the feature matrix to align more than two modalities together.

Our contributions are as follows:
\begin{itemize}
    \item A new singular value based InfoNCE loss to align multiple modalities jointly.
    \item CIPAE learns a joint embedding across RGB images, 2D and 3D human poses.
    \item CIPAE achieves MPJPE $49.4$mm on the Human3.6m dataset and $65.1$mm on the MPI-INF-3DHP dataset.
\end{itemize}

In Sec~\ref{sec:related}, we will discuss related works in 3D HPE, including optimization-based and learning-based methods. In Sec~\ref{sec:method}, details of our backbone architecture and optimization pipeline are addressed. Experimental results are presented in Sec~\ref{sec:exp}, and the ablation study will be discussed in Sec~\ref{sec:discuss}. At last, there are conclusions in Sec~\ref{sec:conclusion}.

==> legacy/3_method.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/poseclip_pipeline.pdf}
    \caption{The training pipeline of CIPAE.}
    \label{fig:pipeline}
\end{figure*}

\section{Methods}
\label{sec:method}


The proposed method aims to eliminate the gap between RGB image, 2D and 3D pose representations and improve the 3D pose estimation accuracy.

As shown in Fig~\ref{fig:pipeline}, for any group of the RGB image, $I \in \mathbb{R}^{h \times w \times 3}$, 2D pose, $P_{2d} \in \mathbb{R}^{J \times 2}$, and 3D pose $P_{2d} \in \mathbb{R}^{J \times 3}$, we want to train Image, 2D and 3D encoders $E_{img}, E_{2d}, E_{3d}$, by maximizing the similarity between image features, $F_{img} \in \mathbb{R}^{n}$, 2D pose features, $F_{2d} \in \mathbb{R}^{n}$, and 3D pose features, $F_{3d} \in \mathbb{R}^{n}$. Meanwhile, 2D and 3D decoders $D_{2d}, D_{3d}$ can estimate corresponding 2D and 3D poses from learned joint embedding.

All the proof of the propositions can be found in the Appendix.

\subsection{CIPAE Encoder}

Following CLIP\cite{radford2021clip}, we have three encoders for three modalities, images, 2D and 3D poses. The encoders, $E_{img}$, $E_{2d}$ and $E_{3d}$ take RGB images, 2D and 3D poses as input and are trained with cosine similarity based InfoNCE\cite{oord2018infonce} loss pairwisely. For any pair of modalities, $\mathcal{S}$ and $\mathcal{T}$, the pairwise InfoNCE loss is

\begin{equation}
    L_{cos} = -\log \frac{\exp{(F_{\mathcal{S}} \cdot F_{\mathcal{T}}^{+} / \tau)}}{\sum_{i=0}^{n}\exp(F_{\mathcal{S}} \cdot F_{\mathcal{T},i} / \tau)},
\end{equation}

where $\tau$ is the learnable temperature.

\begin{figure*}[t]
\begin{minipage}[b]{0.49\textwidth}
\begin{algorithm}[H]
    \centering
    \caption{Random Sampling in $L_{svd}$}\label{algorithm}
    \begin{algorithmic}
        \Require \text{Image features, $F_{img}$ 2D pose}
        \State \text{features, $F_{2d}$, 3D pose features, $F_{3d}$,}
        \State \text{Batch size, $b$} \vspace{5pt}
        \State $\text{index}\_\text{list} \gets \text{zeros}(b, b, 3)$
        \For{$i\gets 0, b$}
        \State $\text{index}\_\text{list}\left[:,i,0 \right] \gets \text{arange}(b)$
        \State $\text{index}\_\text{list}\left[:,0,i \right] \gets \text{arange}(b)$
        \EndFor
        \For{$i\gets 1, b$}
            \For{$j\gets 1, 3$}
                \State $\text{index}\_\text{list}\left[:,i,j \right] \gets \text{shuffle}(\text{arange}(b))$
            \EndFor
        \EndFor
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[b]{0.49\textwidth}
\begin{algorithm}[H]
    \centering
    \caption{Implementation of $L_{svd}$}\label{algorithm1}
    \begin{algorithmic}
        \Require \text{Image features, $F_{img}$ 2D pose}
        \State \text{features, $F_{2d}$, 3D pose features, $F_{3d}$,}
        \State \text{Batch size, $b$, Temperature, $\tau$} \vspace{5pt}
        \State $\mathcal{M}_F \gets \text{stack}((F_{img}, F_{2d}, F_{3d}), dim=1)$
        \State $\text{index}\_\text{list} \gets \text{RandSample}(F_{img}, F_{2d}, F_{3d})$
        \State $\mathcal{M}_F \gets \mathcal{M}_F\left[ \text{index}\_\text{list} \right]$
        \State \text{\# $\mathcal{M}_F \in \mathbb{R}^{b \times b \times 3 \times n}$}
        \State $\mathcal{M}_F \gets \mathcal{M}_F^\intercal\mathcal{M}_F$
        \State $\text{logits} \gets \text{eigenval}(\mathcal{M}_F)\left[:,:,0\right]$
        \State $\text{logits} \gets \text{logits} / \tau$
        \State $\text{label} \gets \text{zeros}(b)$
        \State $L_{svd} = \text{CrossEntropy}(\text{logits}, \text{label})$
        \vspace{9pt}
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\caption{The pseudo-code of group feature random sampling in $L_{svd}$ and the implementation of $L_{svd}$.}
\label{alg:svdloss}
\end{figure*}

In CIPAE, we add one more singular value based InfoNCE loss to learn the joint embedding across three modalities better. For any group of image, 2D and 3D features, features can be stacked as a feature matrix,

\begin{equation}
    F_{img} = \frac{F_{img}}{|F_{img}|}, F_{2d} = \frac{F_{2d}}{|F_{2d}|}, F_{3d} = \frac{F_{3d}}{|F_{3d}|},
    \mathcal{M}_F = 
    \begin{bmatrix}
        F_{img}\\
        F_{2d}\\
        F_{3d}
    \end{bmatrix} \in \mathbb{R}^{3 \times n}.
\end{equation}

According to \cite{MatrixAnalysis}, Singular Value Decomposition (SVD) is a factorization of a real or complex matrix, and the singular values are related to the linear correlation of row vectors. SVD is able to apply to any matrix $\mathcal{M} \in \mathbb{R}^{m \times n}(m \leq n)$,

\begin{equation}
    \mathcal{M} = U\Sigma V^*, U\in \mathbb{R}^{m \times m}, \Sigma \in \mathbb{R}^{m
    \times n}, V \in \mathbb{R}^{n \times n}.
\end{equation}

Diagonal entries, $\sigma_{i}$, in $\Sigma$, are singular values of matrix $\mathcal{M}$, and $\sigma_{1} \geq \sigma_{2} \dots \geq \sigma_{m} \geq 0$. Meanwhile, the number of non-negative singular values is the rank of $\mathcal{M}$.

\begin{prop} \label{prop:singular}
    When all row vectors of a matrix $\mathcal{M}$ are normalized, the square sum of all singular values, $\sigma_i$ of $\mathcal{M}$, is $m$:
    \begin{equation} 
        \sum_{i} \sigma_i^2 = m.
    \end{equation}
\end{prop}

According to Proposition~\ref{prop:singular}, when $\sigma_1 = \sqrt{m}$, the rest of singular values are close to zero, and all row vectors of $\mathcal{M}$ are linearly dependent. Therefore, by maximizing the largest singular values of the feature matrix $\mathcal{F}$, we are able to increase the linear correlations of features from three different modalities,

\begin{equation}
    \argmax_{\sigma_1} \mathcal{F} = U \Sigma V^*.
\end{equation}

However, computing the singular values of $\mathcal{F} \in \mathbb{R}^{3 \times n}$, where $3 \ll n$, is time consuming. In our implementation, the largest eigenvalue $\lambda_1$ of the matrix $\mathcal{F}^T\mathcal{F} \in \mathbb{R}^{3 \times 3}$ is our optimization target, since $\lambda_1 = \sigma_1^2$. In this case, the singular value based InfoNCE loss can be formed as,

\begin{equation}
    L_{svd} = -\log \frac{\exp{(\lambda_1^{+} / \tau)}}{\sum_{i}\exp(\lambda_{1i} / \tau)}.
\end{equation}

However, different from $L_{cos}$, the number of negative samples in $L_{svd}$ is much larger, since in any batch with batch size as $b$, the total number of negative samples is $b^2 - 1$ instead of $b - 1$ in $L_{cos}$. Therefore, we apply a random sampling strategy to ensure there is the same number of negative samples as $L_{cos}$, as shown in~\ref{alg:svdloss}.
  

By maximizing the cosine similarity between positive samples and minimizing the similarity between negative samples, the 2D and 3D encoders are able to align the representations of 2D and 3D poses to the same feature space, as shown in Fig~\ref{fig:intro}. The aligned features can help Action Recognition or Object Tracking pipelines, which bring 3D human pose information to 2D human pose features.

\subsection{CIPAE Decoder}

After the pose features are aligned, we can try two simple decoders for 


==> tab/addition-data.tex <==
\begin{table}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l|cc|cc}
\toprule
 & \multicolumn{2}{c|}{GT 2D} & \multicolumn{2}{c}{Image} \\
Dataset & MPJPE~($\downarrow$)  & PA-MPJPE~($\downarrow$) & MPJPE~($\downarrow$)  & PA-MPJPE~($\downarrow$) \\ 
\midrule
Human3.6M & 39.3 & 29.9 & 58.7 & 44.4\\
Human3.6M + 3DHP & 44.2 & 33.6 & 55.1 & 40.0\\	
\bottomrule
\end{tabular}
}
\caption{\textbf{Ablation study} on training with different datasets. The performance is evaluated on Human3.6m dataset.}
\label{tab:ablation_additional_data}
\end{table}


==> tab/alignment.tex <==
\begin{table}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l|cc|cc}
\toprule
   & \multicolumn{2}{c|}{GT 2D} & \multicolumn{2}{c}{Image} \\
   & MPJPE~($\downarrow$)  & PA-MPJPE~($\downarrow$) & MPJPE~($\downarrow$)  & PA-MPJPE~($\downarrow$) \\ 
\midrule
w/o. & 41.3 & 31.6 & 91.8 &	68.7\\
\rowcolor[gray]{0.9}
w. & 39.3 & 29.9 & 58.7 & 44.4\\	
\bottomrule
\end{tabular}
}
\caption{\textbf{Ablation study} on alignment in 3D HPE task. The performance is evaluated on Human3.6m dataset.}
\label{tab:ablation_alignment}
\end{table}

==> tab/modality-token.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
   & \multicolumn{2}{c|}{GT 2D} & \multicolumn{2}{c|}{DT 2D} & \multicolumn{2}{c}{Image} \\
   & MPJPE~($\downarrow$)  & PA-MPJPE~($\downarrow$) & MPJPE~($\downarrow$)  & PA-MPJPE~($\downarrow$)& MPJPE~($\downarrow$)  & PA-MPJPE~($\downarrow$)\\ 
\midrule
w/o. & 40.9 & 31.7 &	55.0 &	42.7 & 58.7 & 44.4\\
\rowcolor[gray]{0.9}
w. & 39.3 & 29.9 &	53.5 &	40.8 & 57.5	& 42.9\\	
\bottomrule
\end{tabular}
}
\caption{\textbf{Ablation study} on using modality token in 3D HPE task.}
\label{tab:ablation_modality_token}
\end{table}
